Parameter-Efficient Instruction Tuning of Large Language Models For Extreme Financial Numeral Labelling

We study the problem of automatically annotating relevant numerals (GAAP metrics) occurring in the financial documents with their corresponding XBRL tags. Different from prior works, we investigate the feasibility of solving this extreme classification problem using a generative paradigm through instruction tuning of Large Language Models (LLMs). To this end, we leverage metric metadata information to frame our target outputs while proposing a parameter efficient solution for the task using LoRA. We perform experiments on two recently released financial numeric labeling datasets. Our proposed model, FLAN-FinXC, achieves new state-of-the-art performances on both the datasets, outperforming several strong baselines. We explain the better scores of our proposed model by demonstrating its capability for zero-shot as well as the least frequently occurring tags. Also, even when we fail to predict the XBRL tags correctly, our generated output has substantial overlap with the ground-truth in majority of the cases.

==> Sections/zz_HumanEval.tex <==
\subsection{Evaluation by Financial Domain Experts}

%To motivate the difficulty of our problem, we get 
We recruited a team of 6 financial SME who were asked to select the correct label for a numeral in a sentence from a list of top-5 ranked labels by the \axml\ [SHAPE] pipeline model. The experts are of Indian origin and non-native English speakers. They have been working in the industry for an average of 5 years (ranging from 2-10 years). The participants were remunerated equivalent to their half-a-day pay for their involvement in the task. The participants report that they could complete about 30 annotations per hour. It is worth noting that while the team members have an experience of 5 years in the industry on average, they have only a generic knowledge  on XBRL annotation\footnote{The demographic and expertise information, incentives offered are  in the Appendix.}.  
We ensure that the correct label was in the top 5 and this information was revealed to the participants.  In total, 305 datapoints were divided into 3 parts and each part was annotated by 2 SMEs. 
%We find that in total, the annotators were collectively only able to correctly label 375 out of 610 data points (they felt no-confidence for the rest of the points). 

The results, shown in Figure ~\ref{fig:human_performance} show that  the annotators performed best when \axml\ has been able to predict correctly. 
Not only maximum labels were predicted correctly by either both or one of the annotator but the inter-annotator agreement was also high. 
The performance of humans deteriorate a lot for cases where machine has also failed. 

% A team of 6 subject matter experts (SME) were recruited for the evaluation task. 


%This calls for rigorous trainings for humans as well as design of a better human-AI interactive system. 
%Each data point is annotated by 2 participants and we find that only for 59.34\% of the data points were both participants able to correctly classify the datapoints. The overall Inter Annotator Agreement (IAA - $\kappa$ cohen) for these datapoints was 0.658. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.35]{Images/Human Performance hits@k.png}
%     \caption{Hits@k as labelled by annotators}
%     \label{fig:human_performance}
%     %\vspace{-6mm}
% \end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.35]{Images/chart.png}
    \caption{The three bar plots show (a). fraction of times both annotators predicted correctly (b). fraction of correct predictions and (c). inter-annotator agreement for 
     when \axml\ (i). predicted correctly and (ii). failed to predict}
    \label{fig:human_performance}
    %\vspace{-6mm}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.35]{Images/chart (1).png}
%     \caption{Hits@k as labelled by annotators}
%     \label{fig:human_performance}
%     %\vspace{-6mm}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.45]{Images/scatter_random_vs_model.png}
%     \caption{Top-k tag similarity}
%     \label{fig:top_k_tag_sim}
%     %\vspace{-6mm}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.45]{Images/scatter_st_2.png}
%     \caption{Top-k tag similarity \& human agreement}
%     \label{fig:top_k_tag_sim_agreement}
%     %\vspace{-6mm}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.45]{Images/sorted_random_vs_model_agreemnt.png}
%     \caption{Top-k tag similarity \& human agreement}
%     \label{fig:sorted_top_k_tag_sim_agreement}
%     %\vspace{-6mm}
% \end{figure}

==> Sections/zz_Limitations.tex <==
\subsection{Comparison with ChatGPT}

% \section{Limitations}
% This research effort has primarily concentrated on analyzing numerals extracted from 10-K documents, however XBRL annotations are also present in other document types, such as 10-Q quarterly reports. Furthermore, our analysis has been limited to textual data and has not encompassed tabular data. It's worth noting that the process of labeling numerals solely based on individual sentence text can be challenging. Often, the accurate labeling of a numeral necessitates considering the broader context, which could involve examining the surrounding paragraphs, associated tables, and other relevant information. 


% \section{Ethics Statement}
% Given the impact of our proposed contributions on the financial community in particular, and wider research community in general, our dataset and codes wiil be publicly released. Our labels are derived from public/open domain. Still, we may ask users, intending to access our data, to provide a self declaration that the data is to be used solely for research purposes.


\iffalse
\textbf{Contributions}
Our contributions are manifolded.
\begin{itemize}
    \item We first propose a generative approach combined with a matching component to tackle the financial numerical tagging problem, offering a fresh perspective on addressing this complex issue.
    \item  We attain an impressive Hits@1 score exceeding 90\% for an extensive array of labels. This substantially curtail business costs and minimize the investment of man-hours.
    \item The demonstrated Macro-F1 score of ~76\% but also highlights its effectiveness in handling our target labels with heavy-tailed distributions. This offers robustness and reliability of our proposed approach within real-world scenarios and practical business use cases.
    \item Our light weight parameter-efficient model is exceptionally well-suited for deployment and for very quick inference.
\end{itemize}
\fi 

==> Sections/zz_introduction.tex <==
\section{Introduction}

The U.S. Securities and Exchange Commission (SEC) mandates publicly traded companies to disclose periodic filings such as quarterly 10-Q and annual 10-K reports etc.
These documents are of importance to finance professionals and investors who rely on SEC filings to make informed decisions. 
Each company is directed to follow the \textit{Generally Accepted Accounting Principles} (GAAP) to tag numerals appearing in these financial disclosures using \textit{eXtensive Business Reporting Language} (XBRL) according to a well-defined taxonomy consisting of thousands of labels.
Recently, \citet{sharma2023financial} release the \textbf{FNXL} dataset where such numerals are tagged from a large set of 2,794 labels. 
Implementing XBRL tagging therefore requires advanced accounting skills to map financial data to the correct XBRL concepts.
Not only is the task challenging and time-consuming, but hiring experts to meticulously review each document and assign appropriate metric labels is neither a cost-effective nor a scalable solution.
Different from the discriminative approaches explored in prior works \cite{loukas2022finer, sharma2023financial} to solve the task automatically, in this work we present a generative solution for the task of extreme financial numeral labeling by parameter-efficient instruction tuning of Large Language Models (LLMs).

\begin{table}[t]
  \centering
    \resizebox{\linewidth}{!}{
      \begin{tabular}{l|c|c}
        \toprule
        Training Strategies & Macro-F1 \%$\uparrow$ & Hits@1 \%$\uparrow$ \\
        \midrule
        Instruction Tuning Vs. Fine-tuning & 9.5 & 2.7 \\
        Prefix Tuning Vs. Full Instruction Tuning & 5.1 & 5.6 \\
        LoRA Vs. Prefix Tuning & 11.7 & 7.5 \\
        % Training bigger models w/ LoRA & 3.5 & 1.0 \\
        \bottomrule
      \end{tabular} 
      }
   \caption{A systematic comparison of training strategies to improve the performances of \model{} model variants. Reported values represent the \% improvements for models trained with the first strategy over the second strategy.}
   \label{table:flanfinxc_framework}
\end{table}

Among prior works, \textit{\finer{}} \cite{loukas2022finer} formulates the task of identifying relevant numerals from financial texts and tagging them with their appropriate XBRL tags as an NER problem. 
A BERT-based sequence labeling approach is proposed to solve the task.
However, the label set used in \finer{} consists of only 139 most frequently occurring XBRL tags.
For practical purposes however, a significantly larger number of XBRL tags/labels are necessary to effectively annotate the diverse range of numerals present in these documents.
The authors of FNXL dataset \cite{sharma2023financial} explore an extreme classification methodology, \textit{AttentionXML}, to solve the task.
None of these methods however exploit the rich metadata information, readily available with XBRL tags, to improve the classification performance.
\textit{GalaXC} \cite{saini2021galaxc}, on the other hand, is a generic GNN-based extreme classification approach for annotating documents that embeds label metadata information in its document-label graph nodes.
\textit{Label Semantics} \cite{ma2022label} is another generic approach that leverages entity descriptions to solve the standard NER task.
All these methods however lack the capacity to identify unseen labels during inference as they follow a discriminative paradigm.



\begin{figure*}
    \centering     
      % \includegraphics[width=0.9\linewidth]{Images/examples.pdf}
     \includegraphics[width=\linewidth]{Images/annot_example.png}
    \caption{Demonstrating the challenges of solving the Extreme Financial Numeral Labelling task. Within financial statements, one encounters scenarios where all the numerals are associated with distinct XBRL tags, such as in Example 2. Conversely, there are statements where none of the numerals require any tagging, and should instead be designated as \textit{`Others`}, such as in Example 3. Moreover, there are cases where a mixture of both relevant  and irrelevant numerals coexist in the text, often within a very limited context, such as in Example 1. This amalgamation of elements further complicates the accurate tagging process.}

    \label{fig:example}
\pg{Also, can this figure also be used to showcase why tag metadata would actually be helpful? Or bring Table 1 as well, and refer to that from Intro.} \notesk{Table 1 contains the tag doc for common staock shares vs authorized, will refer}
\sg{From Example 3, can there be a risk - readers may just think percentages are Others, so these are easy to classify? \notesk{Right! But for the sentece ` The weighted average target asset allocations at April30, 2021 for the plans are 40\% equity securities, 31\% debt securities, and 29\% other`. For this, all\% numerals getting valid tag--defined benefit plan plan assets target allocation percentage---Should I avoid Example3 and find some other good examples may be}}
\end{figure*}




Generative methods, on the other hand, display intrinsic zero-shot capabilities if trained efficiently.
In this space, LLMs have demonstrated ground-breaking performances across a wide range of NLP tasks in diverse domains \cite{zhao2023survey}, including finance \cite{wu2023bloomberggpt, yang2023fingpt}.
In this work, we solve the task of extreme financial numeral labelling by efficiently training LLMs using \textit{Instruction Tuning}, demonstrated to be a better alternative than old-fashioned fine-tuning for improving the performance and usability of pre-trained LMs \cite{wei2022finetuned}.
More specifically, we instruction tune FLAN-T5 \cite{chung2022scaling} with carefully-curated task specific instructions, as shown in Figure \ref{fig:arch}.
Against prior works for the task \cite{loukas2022finer, sharma2023financial}, we leverage the tag metadata information by using the XBRL tag documentation, instead of the tag themselves, to define our targets for the encoder-decoder FLAN-T5 models.
This decision is driven by our observation that XBRL tags are often very similar to one another differing only in few words, whereas their corresponding documentations allow for a more clear distinction, thereby aiding in the classification task.

\noterm{PG Sir's comments are addressed in the above two paragraphs.}

Through our experiments, we first demonstrate the advantage of training bigger models for the extreme financial numeral labelling task by comparing the results of T5-Large (780M parameters) with T5-Base (220M parameters), achieving \textbf{5\%} Macro-F1 gains and \textbf{2.8\%} Hits@1 gains. 
Next, we demonstrate the advantage of instruction tuning over fine-tuning by comparing the results of FLAN-T5-Large with T5-Large, achieving \textbf{9.4\%} Macro-F1 gains and \textbf{5.6\%} Hits@1 gains.
Given that training larger models is costly, and makes the comparisons with our baselines unfair, next we experiment with parameter-efficient (PEFT) techniques, specifically Prefix Tuning \cite{li2021prefix} and LoRA \cite{hu2021lora}, to instruction tune our FLAN-T5-Large models.
Both techniques require only a small fraction of model parameters to be fine-tuned (0.13\% with Prefix Tuning, and 0.08\% with LoRA), thereby greatly reducing the computation cost and training times. 
Instruction tuning FLAN-T5-large with LoRA outperforms both the Prefix-Tuned version as well as the model variant instruction-tuned without PEFT with \textbf{11.7\%} and \textbf{17.4\%} Macro-F1 gains, respectively.
Our best results are obtained by instruction tuning FLAN-T5-XL (3B parameters) with LoRA (0.08\% of 3B) that outperforms our strongest baseline \textit{AttentionXML} with \textbf{59.4\%} Macro-F1 gains and \textbf{18.3\%} Hits@1 gains, thereby achieving new state-of-the-art results.


\noterm{Working on this...}
We conducted a detailed analysis of our model's performance taking into account the zero-shot scenarios and labels with the least frequent occurrences.  When dealing with labels appearing between 1 to 10 times, we achieved 50\% accuracy in numerical tagging. With number of examples grows to 50, our Hits@1 score rises to 0.77. For few zero shot labels we get F1-score varies in between 0.60 to 0.80 but for some of them we get poor F1-score of 0.30. We also noticed that absence of explicit instruction template(\textbf{14.2\%} drop) or using tag words (XX\% drop) as target significantly impacts the model performance. As the length of the tag documentation, our target, increases, we observed a marginal drop in performance. However, it's worth noting that the LoRA approach consistently maintains a slight edge over the prefix tuning strategy.
\noteng{too much detail -may be avoided.}
Our overall contributions may be summarized as follows:
\begin{itemize}
    \item We first propose a generative approach combined with a matching component to tackle the financial numerical tagging problem, offering a fresh perspective on addressing this complex issue. \pg{Please bring out the novelty. What limitation of the previous approaches have you addressed?}
    \item  We achieve an impressive Hits@1 score exceeding 90\% for an extensive array of labels. The demonstrated Macro-F1 score of ~\textbf{76\%} highlights its effectiveness in handling our target labels with heavy-tailed distributions. 
    \item We excel at efficiently discriminating irrelevant numerals, which should be appropriately tagged as \textit{`others'}. This proficiency holds true even in scenarios where a complex amalgamation of valid taggable numerals coexist within a very limited financial context.

    \item Our light weight parameter-efficient model is exceptionally well-suited for deployment and for very quick inference. \pg{Are we putting the comparisons for this?} \notesk{Yes, we will put \#of params, model size, etc}\pg{Inference time.}
\end{itemize}

\notesk{Add zero shot capability}







==> Sections/zz_tables.tex <==

\iffalse{}
\begin{table}[ht]

\begin{center}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{|p{0.6\linewidth} | p{0.3\linewidth}|}
\hline
\textbf{Dataset}        & \textbf{Entity Types} \\ 
\hline
conll-2003 (Generic) & 4   \\
\hline
ontonotes-v5 (Generic)                & 18                    \\
\hline
ace-2005  (Generic)                   & 7                     \\ 
\hline
genia (Biomedical)                & 36                    \\ 
\hline
\cite{info10080248} (Financial)     & 9                     \\ 
\hline
finer-139 (Financial)                & 139                   \\ 
\hline
\dataset \space(Financial)                 & \textbf{2794}         \\ \hline
\end{tabular}
% }

\caption{\label{table:table_entity_stat}Examples of previous entity extraction
datasets}

\end{center}
\end{table}
\fi




\iffalse
\begin{figure*}[ht]

\centering

\begin{dependency}
\begin{deptext}[column sep=.1cm, row sep=0.3ex]


At April 24, 2020 the estimated fair value was \& \$27.1 \& billion compared to a principal value of \& \$24.5 \& billion.
 \\
\end{deptext}

\wordgroup[group style = {fill = orange!40, draw = red, ultra thick}]{1}{2}{2}{target-gold-1}
\wordgroup[group style = {fill = orange!40, draw = red, ultra thick}]{1}{4}{4}{exp-gold-1}
            
 \groupedge[edge style = {draw = white}, label style = {fill = blue!40}]{target-gold-1}{target-gold-1}{long term debt fair value}{3ex}

 \groupedge[edge style = {draw = brown}, label style = {fill = blue!40, draw = brown}]{exp-gold-1}{exp-gold-1}{debt instrument face amount}{3ex}

\end{dependency}
% \caption{An example sentence with two opinion tuples.}
\label{fig:darmstadt-sample}
\end{figure*}


\begin{figure*}[ht]

\centering

\begin{dependency}
\begin{deptext}[column sep=.2cm, row sep=1.1ex]

Ordinary shares par value\& \$0.0001, \& 2.6 \& billion shares authorized, \& 1,345,400,671 \& and \& 1,341,074,724 \& shares \\ \noindent issued and outstanding, respectively.
 \\ \\ 
\end{deptext}

\wordgroup[group style = {fill = orange!40, draw = red, ultra thick}]{1}{2}{2}{target-gold-1}
\wordgroup[group style = {fill = orange!40, draw = red, ultra thick}]{1}{3}{3}{exp-gold-1}
\wordgroup[group style = {fill = orange!40, draw = red, ultra thick}]{1}{5}{5}{next-gold-1}
\wordgroup[group style = {fill = orange!40, draw = red, ultra thick}]{1}{7}{7}{final-gold-1}
            
 \groupedge[edge style = {draw = brown}, label style = {fill = blue!40, draw = brown}]{target-gold-1}{target-gold-1}{common stock par or stated value per share}{2ex}

 \groupedge[edge style = {draw = brown}, label style = {fill = blue!40, draw = brown}]{exp-gold-1}{exp-gold-1}{common stock shares authorized}{5ex}

 \groupedge[edge style = {draw = brown}, label style = {fill = blue!40, draw = brown}]{next-gold-1}{next-gold-1}{common stock shares issued}{3ex}

 \groupedge[edge style = {draw = brown}, label style = {fill = blue!40, draw = brown}]{final-gold-1}{final-gold-1}{common stock shares issued}{3ex}



\end{dependency}
% \caption{An example sentence with two opinion tuples.}


\label{fig:darmstadt-sample}
\end{figure*}
\fi

